NETCS: A New Simulator of Population Protocols and Network Constructors

Network Constructors are an extension of the standard population protocol model in which finite-state agents interact in pairs under the control of an adversary scheduler. In this work we present NETCS, a simulator designed to evaluate the performance of various network constructors and population protocols under different schedulers and network configurations. Our simulator provides researchers with an intuitive user interface and a quick experimentation environment to evaluate their work. It also harnesses the power of the cloud, as experiments are executed remotely and scheduled through the web interface provided. To prove the validity and quality of our simulator we provide an extensive evaluation of multiple protocols with more than 100000 experiments for different network sizes and configurations that validate the correctness of the theoretical analysis of existing protocols and estimate the real values of the hidden asymptotic coefficients. We also show experimentally (with more than 40000 experiments) that a probabilistic algorithm is capable of counting the actual size of the network in bounded time given a unique leader.

==> schedulers.tex <==

\begin{algorithm}[!h]
  \caption{\emph{Random}}\label{prot:sched:rand}
  \begin{algorithmic}
    \medskip
    \State $N = nodes$

    $initiator$ = select uniformly from $N$
    
    $responder$ = select uniformly from $N-initiator$
    
    interact($initiator$,$responder$)
  \end{algorithmic}
\end{algorithm}
\begin{algorithm}[!h]
  \caption{\emph{History}}\label{prot:sched:hist}
  \begin{algorithmic}
    \medskip
    \State $N = nodes$
    \State $c =$ chance to select a known neighbor

    $initiator$ = select uniformly from $N$
    
    $responder$ = select with chance c from $known$

    $responder$ = select with chance 1-c from $N - initiator - known$
    
    interact($initiator$,$responder$)
  \end{algorithmic}
\end{algorithm}
\begin{algorithm}[!h]
  \caption{\emph{ReverseHistory}}\label{prot:sched:rev}
  \begin{algorithmic}
    \medskip
    \State $N = nodes$
    \State $c =$ chance to select an unknown neighbor

    $initiator$ = select uniformly from $N$
    
    $responder$ = select with chance c from $N-initiator- known$

    $responder$ = select with chance 1-c from $known$
    
    interact($initiator$,$responder$)
  \end{algorithmic}
\end{algorithm}
\begin{algorithm}[!h]
  \caption{\emph{Connection}}\label{prot:sched:rev}
  \begin{algorithmic}
    \medskip
    \State $N = nodes$
    \State $c =$ chance to select a neighbor with an active connection

    $initiator$ = select uniformly from $N$
    
    $responder$ = select with chance c from $active$

    $responder$ = select with chance 1-c from $N-initiator- active$
    
    interact($initiator$,$responder$)
  \end{algorithmic}
\end{algorithm}
